Utilizing Every Image Object for Semi-supervised Phrase Grounding

Phrase grounding models localize an object in the image given a referring expression. The annotated language queries available during training are limited, which also limits the variations of language combinations that a model can see during training. In this paper, we study the case applying objects without labeled queries for training the semi-supervised phrase grounding. We propose to use learned location and subject embedding predictors (LSEP) to generate the corresponding language embeddings for objects lacking annotated queries in the training set. With the assistance of the detector, we also apply LSEP to train a grounding model on images without any annotation. We evaluate our method based on MAttNet on three public datasets: RefCOCO, RefCOCO+, and RefCOCOg. We show that our predictors allow the grounding system to learn from the objects without labeled queries and improve accuracy by 34.9\% relatively with the detection results.

==> sections/2-intro-old.tex <==
The task of phrase grounding is to localize entities referred to by the given natural language phrases.
This requires associating words and phrases from language modality to objects and relations in the visual modality.
Grounding plays an important role in the applications for language and vision, such as visual question answering \cite{antol2015vqa,das2018embodied,gordon2018iqa,li2018attentive,zhang2019interpretable}, image retrieval \cite{wang2018joint} and captioning \cite{anderson2018bottom,vinyals2015show}. 

It is not reasonable for a grounding system to have encountered all potential combinations of words in noun phrases. A grounding system needs to localize queries containing novel combinations;  thus,  transfer of attributes and relations from one category to another is essential. 
Modern grounding systems, such as MAttNet \cite{yu2018mattnet}, do have such capabilities, but they are trained under fully supervised settings where every object used in training has a corresponding query (i.e., a text description)  in the training set. This limits the data used for training, where only images with dense annotations can be used. Fig.~\ref{fig:grounding example} shows two examples where not all objects are annotated. 

%It is not reasonable for a grounding system to have encountered all potential combinations of words in noun phrases. A grounding system needs to localize queries containing novel combinations;  thus, the transfer of attributes and relations from one category to another is essential. 
%Modern grounding systems, such as MAttNet \cite{yu2018mattnet}, do have such capabilities, but they are trained under fully supervised settings where every object used in training has a corresponding query (i.e., a text description)  in the training set. This limits the data used for training, where only images with dense annotations can be used.

Unlike previous semi-supervised grounding systems \cite{rohrbach2016grounding,liu2019knowledge}, which still require full query annotation for the objects in the unlabeled images in the training set, our method can directly be trained on the images without any annotations except the detection results from the detector.
%{\red 
%Existing semi-supervised methods are not feasible for the settings where full query annotations are not available during training, since they cannot extract other information other than the category names from the unlabeled images. 
%A query in a grounding dataset uniquely identifies an instance of a category; category name alone does not perform such discrimination and is thus not effective if used to train a model in fully supervised manner.}
The queries in grounding datasets are discriminative within a category, whereas the category names along do not perform such discrimination compared with the whole query. Thus it is not effective by simply applying the category names as the full query for training the grounding model as what is done by other semi-supervised methods.

%The queries in grounding datasets are  discriminative within a category, whereas the category names do not bring distinctions more than a classifier, which makes it doesn't improve the accuracy of the grounding model when simply using the category name as the full query to train the model as the fully supervised setting.
%A straightforward modification of the supervised method is to use the category names as queries associated with the object for training. However, we find that such augmentation actually does not improve the accuracy of the grounder; a possible explanation for this is that the queries in grounding datasets are highly discriminative within a category whereas the category name cannot bring distinctions more than a classifier. 


%Moreover, inappropriate using the unlabeled objects as a negative example can cause extra confusion to the grounding model. For example, in Fig.~\ref{fig:grounding example} (b) if we use the dog in the green box as a negative example for the query `\textit{white dog lying on the grass on the left}', the grounding model will not be able to distinguish about which part in the query is not matching with the object, `white', `dog', `lying on the grass' or `on the left'.
%A grounding model can see the noun and its attribute separately, but a specific combination for the noun with such attributes may not be seen. 
%We show two examples in Fig.~\ref{fig:grounding example}.
%The first example is the new combination of the existing category, while the second example is attaching the attribute into a new category.
%{\color{red} ExEP-Netd on this, two examples are of different style } 
%The ability of the model is limited by the specific combinations it has seen during training.
%During training, the model is familiar with `blue \textit{car}' and `\textit{red} sofa'. 
%But when we ask the model to ground a `red car', the grounding model cannot locate it correctly.
%In the meantime, for a new category with its name available only, or for an object which has not even one word given as the label, current phrase grounding methods suffer to recognize a. 
%Existing phrase grounding methods suffer when facing such query combinations, since they cannot hand. 
%{\color{red} Are they not designed to handle such queries or just not evaluated in this setting? } % and objects without proper queries.
%Also, if we add a new category to the existing dataset with its category name and detection results only, current methods will face trouble to transform existing attributes to this new category. 

%\resizebox{.99\columnwidth}{!}{

\begin{figure}
    \centering
    \begin{tabular}{cc}
        \includegraphics[width=0.45\linewidth]{images/new_new_street.jpg} & 
        \includegraphics[width=0.45\linewidth]{images/new_new_multidog.jpg} \\
         (a) &
        (b) \\
        
    \end{tabular}%
    % }
    
    \par%\smallskip
    \caption{We may have some images in the training set where only some of the objects (those shown in red boxes) are labeled. Red boxes in the two images are annotated as `\textit{black car}' and `\textit{white dog lying on the grass on the left}' respectively, while objects in green boxes only have bounding boxes and category names, `\textit{car}' and `\textit{dog}', associated with them.}
    \label{fig:grounding example}
\end{figure}

We propose to train modules that predict query embedding features from visual embedding features when the associated objects do not have associated descriptive phrases. 
In particular, we include two embedding predictors to encode properties of the subject and location of the objects from the given images. 
The predicted features are then combined with visual features to compute a grounding score. We expect the predicted embeddings to be not perfect but still useful in improving training. 
The embedding predictors themselves are also trained in an end-to-end framework; we call the resulting modules to be  Location and Subject Embedding Predictors, abbreviated as LSEP. 
Note we apply the LSEP modules in the training phase only, since we always have the specified query during inference.

% Our method builds on MattNet architecure \cite{ yu2018mattnet} and our predictor modules replace the query encoding algorithms in MattNet. 

We test the utility of LSEP in several different settings, including cases where the unannotated objects come from the same or different images, and where some object categories are never seen with query phrases in training. 
We create these settings by taking subsets of three commonly used datasets: RefCOCO \cite{yu2016modeling}, RefCOCO+  and RefCOCOg \cite{mao2016generation}. 
We use MAttNet  \cite{ yu2018mattnet} as our base architecture and observe consistent improvement by adding LSEP modules during training. 
%Furthermore, even under a worse circumstance, where some bounding boxes come from a detector instead of ground truth, LSEP shows consistent improvement in semi-supervised phrased training.
%Furthermore, LSEP shows consistent improvement in semi-supervised phrased training using bounding boxes from a detector instead of groundtruth annotations when annotated queries are missing.
Furthermore, when both the groundtruth bounding boxes and queries are not available, LSEP still shows consistent improvement in semi-supervised phrased training by using bounding boxes predicted by a detector.

%We also show the consistent improvement for using LSEP in semi-supervised phrased training with a detector, where no annotations, including groundtruth bounding boxes, are available for some images in the training set.

%over the same network without the embedding predictors; this allows the system to learn to ground new categories given a detector for such categories.

 
In summary, our contributions are three-fold: 
{
(i) we introduce a new semi-supervised setting for phrase grounding training  with limited labeled queries, and we create four sub-settings,
(ii) we propose subject and location embedding predictors for generating corresponding language features from the visual information to narrow the gap between supervised and semi-supervised tasks, and 
(iii) we extend the training of a semi-supervised phrase grounding model to unlabeled images using a pretrained detector.
}
%we show that our method narrows the gap between semi-supervised and supervised tasks for phrase grounding with attribute transfer between different queries.
 
%In the following sections, we will first introduce related work, then introduce our model with its implementation details, followed by the experiments and results on public datasets.



==> sections/3-related.tex <==
\textbf{Phrase Grounding} has been largely studied under the supervised formulation where query annotations are paired with the bounding boxes in the image.
On popular phrase grounding datasets like RefCOCO \cite{yu2016modeling, mao2016generation} and Flickr30k Entities \cite{flickrentitiesijcv, flickr30k}, state-of-the-art methods \cite{yu2018mattnet,Chen2017QueryGuidedRN} use a two-step process: find all the objects using an object detector and then jointly reason over the query and the detected objects.
Recently, single-stage grounding methods \cite{Yang2019AFA,sadhu2019zero}, where both steps are combined, have shown better performance on RefClef \cite{kazemzadeh2014referitgame}.
In our work, we build on MattNet \cite{yu2018mattnet} to enable semi-supervised learning.


These models are pretrained on a large paired image-caption data like conceptual captions \cite{Sharma2018ConceptualCA} or aggregated vision+language datasets \cite{tan2019lxmert}.
As a result, it is difficult to evaluate them in the semi-supervised setting whose language annotations are scarce.

\textbf{Semi-Supervised Phrase Grounding} where language annotations are scarce has not been explored but there are some closely related publications.  
GroundeR \cite{rohrbach2016grounding} considers semi-supervised localization where both language annotations and bounding boxes are present, however, the association is provided only for a subset.
Zero-Shot Grounding (ZSG) \cite{sadhu2019zero} in contrast explores grounding of novel objects for which bounding boxes are never seen during training.
Our proposed formulation lies somewhere in between: we assume object bounding boxes are known, but language annotations are not given. 
%As such, it can be considered a relaxed version of ZSG.





==> sections/6-result-old.tex <==

\subsection{Results and Analysis}
%In this subsection, we will show the results for implementing the transformer to the MAttNet \cite{yu2018mattnet} with other baseline methods for all our three settings. We will first compare our method on supervised learning problem 
In this subsection, we first show quantitative results for four semi-supervised settings  with different ratios of annotations, followed by the results using a detector instead of the groundtruth bounding boxes and some ablations.







%Results are shown in Table~\ref{table:fsg}. 
%We compared our method with seven state-of-the-art methods, including MAttNet \cite{yu2018mattnet}. 
%Compared with other state-of-the-art methods, our model outperforms other methods on all three datasets. Note that with the same amount of annotations, our model can still get better results than the original MAttNet \cite{yu2018mattnet} model. The result shows that with the same amount of annotation, we can utilize more information from the unannotated visual information and apply it for a better grounder.


\input{tables/acc_f1_categ}

\textbf{Semi-supervised grounding results}\label{semisup}
%In semi-supervised part, we follow Sec.~\ref{dataset} to build four different settings for semi-supervised grounding. 
We first show results for four different selection settings in Table~\ref{table:zsl}. We set all these four settings to be 50\% labeled with queries, while the other 50\% have the category names only.
%We follow the MAttNet to first use the annotated groundtruth bounding box for every object and match it with the given query during inference.
We follow the MAttNet to match the given query with every annotated groundtruth bounding boxes in the image and pick the one with the highest score as the final prediction. 
We observe that, for annotation, image, and category-based selections, LSEP outperforms MAttNet on most of the splits for all three datasets, while the accuracy for the supercategory-based is almost the same. 
Comparing the F1 results between category and supercategory-based selection settings, we show that the grounding model can apply features from a nearby category, even labels for such categories are not available, since the objects in the same supercategory share similar visual features. 
F1 scores for all these four settings improve to a relatively significant extent, indicating that the final attribute accuracy improves with our subject embeddings predictor. 
Better F1 results for all four selection settings show that LSEP enables better attribute combinations transfers from labeled queries in the training set to unseen combinations compared with MAttNet.

{\red

{ 
We analyze the performance with different ratios of annotated queries, and investigate whether using the category name as the labeled query in the training stage is helpful in Table~\ref{table:ssl-ab}. 
%\textbf{Supervised grounding results}\label{supervised}
We first show some comparisons when the labeled ratio is 100\% with some other fully supervised phrase grounding methods.
We use the bounding boxes from the groundtruth annotations of the MSCOCO dataset as candidate proposals. 
During training, every bounding box is equipped with a descriptive query.
For LSEP, we first train the two predictors with these groundtruth annotations. We then use these two language encoders to generate corresponding embeddings from the encoded visual embeddings and apply them for training the grounding model.
%By applying the same back-bone network, our model outperforms 
Our model shows similar state-of-the-art performance and even outperforms MAttNet on some splits.
%Our model outperforms most of the splits in all three datasets compared with other state-of-the-art grounding methods, and even better than the original MAttNet. 
The generated embeddings are powerful in training a good grounding model, and LSEP, compared with a fully supervised method, can extract further information besides the queries given in the annotations and sightly improve the performance for phrase grounding when all queries are available. 

%Based on the results where 100\% annotations are available, we compare this baseline with three different ratios of unlabeled images for annotation-based and image-based selection settings.
We then remove part of the labeled queries and set three different ratios of unlabeled images for annotation-based and image-based selection settings.
We observe that, with fewer available annotations in the training set, the performances for both MAttNet and LSEP go down. Still, LSEP can narrow the gap by around $40\%$ between training the grounding model on partially and fully labeled data. 
We also find that the accuracy for the image-based selection setting is higher compared with the annotation-based selection setting when the number of available queries is limited to the same level. 
This indicates that densely-annotated images help a grounding model find the differences between objects; objects in the same image create more challenging object-query pairs for the phrase grounding model to distinguish the subtle differences in the same surroundings and circumstances. 
By comparing the results of whether using the category names or not as the labeled query for training, we find the performances of these two are similar, which indicates that using the category name as the full query does not improve the grounding accuracy. This is because if using the category name as the full query during training, we need to ensure that negative examples are not from the same category. For example, if we use the annotated query or the generated language embedding from the embedding predictors, a 'black cat' can be treated as a negative example of a 'white cat'; however, this is not the case when using only the category name as both are cats. 
Compared with distinguishing two objects belonging to the same categories, using two different objects from different categories shows limited benefit since the grounding model can easily distinguish two objects from their category.
%This also shows that 
%distinguishing the objects belonging to different categories on the extra images doesn't significantly help the phrase grounding task.
%{\color{red} This sentence not very clear } . 
%The model learns more from hard example pairs and finds out the subtle differences between different proposals.
%{\color{red} This para should include some quantitative analysis, not just refer to the Table. } 

}
%{\color{red} Improvement is not so clear, maybe better to say results are similar? } 

%We are able to extract supervised
}

\input{tables/semi_result}

\textbf{Semi-supervised phrase grounding with detector} { 
Instead of using MSCOCO groundtruth boxes, we further compare the semi-supervised phrase grounding results with the proposals generated by a pretrained detector. We use the image-based selection as the experiment setting, and set the percentage of images that have been annotated as 50\% for all configurations. We use a Faster R-CNN \cite{ren2015faster} trained on MSCOCO 2014 \cite{lin2014microsoft} detection task provided by MAttNet \cite{yu2018mattnet} as our detector. During training, we use the proposal with the maximum IoU with the groundtruth bounding box for those objects with labeled queries. For the remaining 50\% that are unlabeled with any query, we use the detection results and their category names provided by the detector. For inference, we select among the detected bounding boxes generated by the Faster R-CNN. We show the grounding accuracy on all three datasets in Table~\ref{table:detect} with the fully supervised results for comparison, where all queries are available. {\red By comparing the gap between supervised results of MAttNet and the settings when labeled bounding boxes are limited, we find that the grounding accuracy is relatively 34.9\% better on average when using LSEP for predicting the query embeddings and consistent improvement for all three datasets.} Results show that by using a pretrained detector, we can apply LSEP for extracting information to learn from the images without any annotations in addition to the labeled proposals.} %This shows that with the detection result of the extra image, we can improve the performance of the model without any extra need for human annotations.

\begin{figure*}
    \centering\resizebox{.99\linewidth}{!}{
    \begin{tabular}{cccc}
    
        \includegraphics[width=0.25\linewidth]{images/refcocog_umd_val_00083.png} & 
        \includegraphics[width=0.25\linewidth]{images/refcocog_umd_val_00083_the_donut_in_the_front.png} & 
        \includegraphics[width=0.25\linewidth]{visresult/refcocog_umd_val_00122.png} & 
        \includegraphics[width=0.25\linewidth]{visresult/refcocog_umd_val_00122_a_white_and_blue_bag_on_top_of_a_black_suitcase.png} 
        \\
        \multicolumn{2}{c}{(a) The donut in the front} & \multicolumn{2}{c}{(b) A white and blue bag on top of a black suitcase}\\
        
       \includegraphics[width=0.25\linewidth]{visresult/new_refcoco_unc_val_00020.jpg} & 
        \includegraphics[width=0.25\linewidth]{visresult/new_refcoco_unc_val_00020_third_bottle_from_the_left.jpg} & 
        \includegraphics[width=0.25\linewidth]{visresult/new_refcoco_unc_val_00085.jpg} & 
        \includegraphics[width=0.25\linewidth]{visresult/new_refcoco_unc_val_00085_second_stack_of_<UNK>_from_right.jpg} 
        \\
        \multicolumn{2}{c}{(a) Third bottle from the left} & \multicolumn{2}{c}{(b) Second stack of $<$UNK$>$ from right}
        \\
        
        \includegraphics[width=0.25\linewidth]{visresult/refcoco_unc_val_00030.png} & 
        \includegraphics[width=0.25\linewidth]{visresult/refcoco_unc_val_00030_the_right_half_of_the_left_sandwich.png} & 
        \includegraphics[width=0.25\linewidth]{images/refcoco_unc_val_00176.png} & 
        \includegraphics[width=0.25\linewidth]{images/refcoco_unc_val_00176_chair_her_foot_is_on.png} 
        \\
        \multicolumn{2}{c}{(c) The right half of the left sandwich} & \multicolumn{2}{c}{(d) Chair her foot is on}
        \\
        
        
        \includegraphics[width=0.25\linewidth]{visresult/new_refcocog_umd_val_00135.jpg} & 
        \includegraphics[width=0.25\linewidth]{visresult/new_refcocog_umd_val_00135_the_giraffe_whose_head_is_not_visible.jpg} & 
        \includegraphics[width=0.25\linewidth]{visresult/new_refcoco_unc_val_00011.jpg} & 
        \includegraphics[width=0.25\linewidth]{visresult/new_refcoco_unc_val_00011_right_side_second_banana_up.jpg} 
        \\
        \multicolumn{2}{c}{(c) The giraffe whose head is not visible} & \multicolumn{2}{c}{(d) Right side second banana up}
        \\
       
        
    \end{tabular}%
     }
    
    \par\bigskip
\caption{Visualization results. The images on the left are the results for MAttNet and images on the right are the results for LSEP.}
\label{fig:vis}
\end{figure*}


\textbf{Ablation study} 
%To evaluate the performance of our two proposed modules, we perform an ablation study to verify how the influence of the two separately.
We conduct an ablation study about how much the two embedding predictors contribute to the improvement of semi-supervised grounding accuracy.
We use the RefCOCO dataset with 50\% annotations available based on annotation-based selection. 
%We made a comparison for LSEP and two modules independently with MAttNet. % since RefCOCO includes both annotations for location and other attributes. 
%We also make a comparison between the original MAttNet that only uses bounding boxes for the remaining unlabeled objects and the one uses both category names along with the bounding boxes. %method $o_k$ from all the available bounding boxes (denoted as MAttNet) and only from the objects with labeled queries (denoted as MAttNet*).
We show the results in Table~\ref{table:ablation}. We observe that both the subject and location embedding predictors improve the grounding accuracy, and the combination of two predictors has the highest score.
Both subject and object predictors help with better grounding results compared with original MAttNet.
%Moreover, by comparing MAttNet using category names as positive labels or not during training, we found that the one not using category names to make these unlabeled objects as positive examples makes no big difference compared with the one uses. 
%This shows that using extra annotations with category names only actually doesn't provide the distinctions that a grounding system needs, which also shows the validity for us not using category names in MAttNet for the annotation and image-based settings. %Since we are introducing new categories in the category and supercategory-based settings, category names are necessary and cannot be discarded in the experiment. 
%Moreover, by comparing MAttNet and MAttNet* on testA and testB, we also found that the grounding accuracy reduces on category `person', which dominants the whole dataset, and improves on most of the other categories after using extra bounding boxes as negative examples. This shows that when training examples are adequate, negative examples that are not used as positive ones harm the performance of the final grounding result, while extra information for the categories with few objects improves its performance.

%Since only RefCOCO \cite{yu2016modeling} contains both attribute and location descriptions in the queries; we evaluate the performance of the two modules when 50\% of annotations are not available. 
%The annotation selection strategy is random on annotation id. Results are shown in Table~\ref{table:ablation}.

\input{tables/detect_bbox}


\subsection{Qualitative Results}\label{qualitative}
We show some visualization results in Fig.~\ref{fig:vis}. 
Results in the four rows are for annotation-based, image-based, category-based and supercategory-based selection settings respectively.
%Results in the first row are for the image-based selection setting, and in the second row are for categories without full queries in the category-based setting. 
%Result on the left are the 
We show the grounding results for MAttNet of the same pair on the left and LSEP on the right.
Results shown for the category-based and supercategory-based selection settings are the categories whose full queries are not available during training.
We find that MAttNet successfully finds the object of the same category, such as the `bottle' in the first example of the second row, but it fails to find the one based on the given query, while LSEP successfully localizes the third bottle from the left in the image. %With the successful transfer from other queries, LSEP is able to handle the grounding case for both seen and unseen categories.

%The four rows shows the original grounding result
%We plot our visualization results in Fig.~\ref{fig:vis}. The first two columns compare the grounding results for semi-supervised learning with the original method and the last two rows shows the results for zero-shot compared with original grounding result. 
%With the prediction alignment module applied, the zero-shot method can be more applied for more difficult circumstances. 
%Also, with the transformer, the grounder can successfully transfer the attribute from a known category to an unknown category to help built the overall accuracy.


%From the table we can tell that with either of the proposed module, our model can outperform the original mattnet model. 
%When we use both of these two modules, the final accuracy is higher than just one of them, showing both of the module contribute when location or attribute features are generated.


\input{tables/abla_one_line}


==> tables/abla.tex <==

\begin{table}[]
\begin{center}
\resizebox{.99\columnwidth}{!}
{
\begin{tabular}{p{4.5cm}p{0.0cm}<{\centering}p{0.9cm}<{\centering}p{0.9cm}<{\centering}p{0.9cm}<{\centering}}
\toprule
Acc&& Val & testA & testB \\
 \midrule
MAttNet           &  &79.33& 80.07 &78.05 \\      
MAttNet + subject translator      &  &  80.85  & 82.09 &  79.57   \\      
MAttNet + location translator      &&   80.98    &   81.81    &   78.88   \\      
LSEP   &  &\textbf{82.11}&\textbf{83.60} &\textbf{80.96}   \\  
\bottomrule
\end{tabular}
}
\end{center}
\caption{Ablation study for module evaluation}
\label{table:ablation}
\end{table}


==> tables/ann_img_sel.tex <==

\begin{table*}[]
\begin{center}
%\resizebox{.97\columnwidth}{!}
{
\begin{tabular}{p{1.45cm}p{2.65cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.0cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.0cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}}
\toprule
 &Type /&\multicolumn{3}{c}{RefCOCO}
 && \multicolumn{3}{c}{RefCOCO+}
 && \multicolumn{2}{c}{RefCOCOg} \\ 
% \midrule
\cline{3-5}\cline{7-9}\cline{11-12}\\[-8pt]
 & Labeled \% & Val  &  testA & testB&& Val &testA &testB && Val & testA   \\ \midrule   
MAttNet &annotation-75\%&81.78& 83.54 &79.26 &&61.08& 64.83& 56.58 && 72.14 & 72.07 \\ 
LSEP &annotation-75\%&\textbf{83.02}&\textbf{84.70} &\textbf{79.60} &&\textbf{67.53}& \textbf{70.07}& \textbf{61.51 }&& \textbf{75.53} & \textbf{74.82} \\ 
\midrule         
MAttNet &annotation-50\%&79.33& 80.07 &78.05 &&55.59& 60.95& 49.46 && 71.20& 70.75\\   
LSEP &annotation-50\%&\textbf{82.11}&\textbf{83.60} &\textbf{80.96} && \textbf{60.28}& \textbf{65.19}& \textbf{53.18} && \textbf{73.71}& \textbf{72.93}\\ 
\midrule         
MAttNet &annotation-25\%&63.73& 66.01 &62.88& &42.96& 48.10& 39.76 && 67.10 & 67.13 \\ 
LSEP  &annotation-25\%&\textbf{67.43}& \textbf{70.55} &\textbf{66.01} & &\textbf{46.94} &\textbf{52.81} & \textbf{41.42} && \textbf{69.08} & \textbf{69.52} \\        
\midrule
MAttNet &image-75\%& 82.89& 83.45 &81.51 &&68.40& 71.18& 64.14 & & 75.76  & 75.32  \\      
LSEP &image-75\%&\textbf{83.70}& \textbf{84.38} &\textbf{82.85} &&\textbf{70.12}& \textbf{73.05}& \textbf{64.59} && \textbf{75.94} & \textbf{76.15} \\  
\midrule
MAttNet&image-50\%&82.40& 83.33 &80.79 &&67.42& 70.19& 61.96 && 74.61 & 73.65\\  
LSEP &image-50\%&\textbf{83.34}& \textbf{83.54} &\textbf{82.16} &&\textbf{68.85}& \textbf{71.08}& \textbf{63.31} && \textbf{75.94}& \textbf{75.35}\\ 
\midrule             
MAttNet &image-25\%& 79.92 & 80.25   &78.81 && 63.90 & 66.92   &59.85 &&68.34  &68.20\\ 
LSEP&image-25\%& \textbf{82.32} & \textbf{82.77}& \textbf{80.48 } & &\textbf{67.22} & \textbf{69.80}  & \textbf{62.38}& & \textbf{73.14} &\textbf{72.42}\\  
\bottomrule
\end{tabular}}
\end{center}
\caption{Semi-supervised results for grounding for annotation-based and image-based selections. The number after dash represent the percentage of bounding boxes that has been labeled with queries during training.}
\label{table:ssl-ab}
\end{table*}


==> tables/sup_tab.tex <==

\begin{table*}[t]
\begin{center}
%\resizebox{.99\linewidth}{!}
{
\begin{tabular}{p{2.395cm}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.0cm}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.0cm}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}}
\toprule
 & \multicolumn{3}{c}{RefCOCO}
 && \multicolumn{3}{c}{RefCOCO+}
 && \multicolumn{3}{c}{RefCOCOg} \\ 
%    \midrule
\cline{2-4}\cline{6-8}\cline{10-12}\\[-8pt]
& val  & testA &   testB  && val &  testA  &  testB  && val* & val & test        \\ 
\midrule
%MMI \cite{mao2016generation}&-&71.72&71.09&&-&58.42&51.23&&62.14&-&-\\ 
%NegBag \cite{nagaraja2016modeling}&76.90 & 75.60 & 78.00 &&- & -& - &&-&- &68.40\\ 
%visdif+MMI \cite{yu2016modeling}&- & 73.98 & 76.59& &- & 59.17& 55.62 && 64.02& -&-\\ 
%Luo et al. \cite{luo2017comprehension}&- & 74.04 & 73.43 &&- & 60.26& 55.03& & 65.36& -&-\\ 
%CMN \cite{hu2017modeling}& - & - & - && - & -& - && 69.30& -&-\\ 
%visdif \cite{yu2016modeling}& 76.08 & 74.39 & 77.30 && 58.94 & 61.29& 56.24 && 59.40& -&-\\ 
%S-L-R \cite{yu2017joint}& 79.56 & 78.95 & 80.22 && 62.26 & 64.60 & 59.62 && 72.63& 71.65&71.92\\ 
%VC \cite{zhang2018grounding}&- & 78.98 & 82.39 &&- & 62.56& 62.90 && 73.98& -&-\\ 
%Attr \cite{liu2017referring}&- & 78.05 & 78.07 &&- & 61.47& 57.22 && 69.83& -&-\\ 
Accu-Att \cite{deng2018visual}& 81.27 & 81.17 & 80.01 && 65.56 & 68.76 & 60.63 && 73.18& -&-\\ 
 PLAN \cite{zhuang2018parallel}&81.67 & 80.81 & 81.32 &&64.18 & 66.31& 61.46 && 69.47& -&-\\ 
Multi-hop \cite{strub2018visual}& 84.90 & 87.40 & 83.10 &&73.80 & 78.70& 65.80 && 71.50& -&-\\ 
MAttNet \cite{yu2018mattnet}& 85.65 & 85.26 & \textbf{84.57} && 71.01 & 75.13 & 66.17 && - & 78.10 & 78.12\\ 
\midrule
LSEP &\textbf{85.71}& \textbf{85.69} & 84.26 &&\textbf{71.99}& \textbf{75.36}& \textbf{66.25}&& -  & \textbf{78.96}&\textbf{78.29}\\ 
\bottomrule
\end{tabular}
}
\end{center}
\caption{Experiment of phrase grounding results on groundtruth MS COCO regions.}
\label{table:fsg}
\end{table*}



==> tables/tmp_acc_f1_merged.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \begin{table}[]
% \footnotesize
% \resizebox{0.5\textwidth}{!}{%
% \begin{tabular}{cccccccccc}
% Val            & testA          & testB          &  & Val            & testA          & testB          &  & Val            & test           \\
% 33.05          & 32.84          & 34.89          &  & 21.25          & 15.38          & 22.17          &  & 25.91          & 23.44          \\
% \textbf{36.41} & \textbf{40.58} & \textbf{35.89} &  & \textbf{24.79} & \textbf{17.39} & \textbf{26.14} &  & \textbf{32.86} & \textbf{32.08}
% \end{tabular}%
% }
% \caption{}
% \label{tab:my-table}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \begin{table}[]
% \resizebox{0.5\textwidth}{!}{%
% \begin{tabular}{cccccccccccc}
%         &   & Val            & testA          & testB          &  & Val            & testA          & testB          &  & Val            & test           \\
% MAttNet & C & 33.05          & 32.84          & 34.89          &  & 21.25          & 15.38          & 22.17          &  & 25.91          & 23.44          \\
% PAN  & C & \textbf{36.41} & \textbf{40.58} & \textbf{35.89} &  & \textbf{24.79} & \textbf{17.39} & \textbf{26.14} &  & \textbf{32.86} & \textbf{32.08}
% \end{tabular}%
% }
% \caption{}
% \label{tab:my-table}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \begin{table}[]
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{cccccccccccccccccccc}
%         &   & \multicolumn{2}{c}{V}           & \multicolumn{2}{c}{TA}          & \multicolumn{2}{c}{TB}          &  & \multicolumn{2}{c}{V}           & \multicolumn{2}{c}{TA}          & \multicolumn{2}{c}{TB}          &  & \multicolumn{2}{c}{V}           & \multicolumn{2}{c}{T}           \\
%         &   & A              & F1             & A              & F1             & A              & F1             &  & A              & F              & A              & F              & A              & F              &  & A              & F              & A              & F              \\
% MattNet & C & \textbf{71.71} & 33.05          & 69.68          & 32.84          & 73.97          & 34.89          &  & 50.51          & 21.25          & 44.00          & 15.38          & 49.68          & 22.17          &  & 59.82          & 25.91          & 60.34          & 23.44          \\
% PAN  & C & 71.64          & \textbf{36.41} & \textbf{72.90} & \textbf{40.58} & \textbf{75.18} & \textbf{35.89} &  & \textbf{51.73} & \textbf{24.79} & \textbf{47.33} & \textbf{17.39} & \textbf{52.91} & \textbf{26.14} &  & \textbf{63.90} & \textbf{32.86} & \textbf{63.41} & \textbf{32.08}
% \end{tabular}%
% }
% \caption{}
% \label{tab:my-table}
% \end{table}

% \begin{table}[]
% \begin{center}
% \resizebox{.99\columnwidth}{!}
% {
% \begin{tabular}{p{1.395cm}p{1.8cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.0cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.0cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}}
% % \toprule
%  Grounding&&\multicolumn{3}{c}{RefCOCO}
%  && \multicolumn{3}{c}{RefCOCO+}
%  && \multicolumn{2}{c}{RefCOCOg} \\ 
% % \midrule
% % \cline{3-5}\cline{7-9}\cline{11-12}\\[-8pt]
% Accuracy& type&Val & testA& testB &&Val& testA&testB &&Val& test  \\ 
% % \midrule   
% MAttNet & category &\textbf{71.71}  & 69.68 &73.97 &&50.51  &44.00  &49.68  && 59.82 & 60.34\\
% PAN &category &71.64  & \textbf{72.90}   &\textbf{75.18} &&\textbf{51.73} &\textbf{47.33} & \textbf{52.91} &&  \textbf{63.90}  & \textbf{63.41} \\
% % \midrule
% MAttNet & supercategory & \textbf{70.59} & 58.89  &\textbf{73.18} &&48.54  &\textbf{39.23}  &\textbf{50.27} &&  \textbf{56.88} & \textbf{54.31} \\
% PAN & supercategory &68.80  &\textbf{60.00}  &72.01&&  \textbf{48.61}  & 38.67 & 50.16&& 56.54 & 53.93 \\ 
% % \midrule
% \end{tabular}
% }
% \resizebox{.99\columnwidth}{!}
% {
% \begin{tabular}{p{1.395cm}p{1.8cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.0cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.0cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}}
% % \midrule
%  F1&&\multicolumn{3}{c}{RefCOCO}
%  && \multicolumn{3}{c}{RefCOCO+}
%  && \multicolumn{2}{c}{RefCOCOg} \\ 
% % \midrule
% \cline{3-5}\cline{7-9}\cline{11-12}\\[-8pt]
% score & type&Val & testA& testB &&Val& testA&testB &&Val& test  \\ 
% % \midrule
% MAttNet & category &33.05  &  32.84 &34.89 & & 21.25 &15.38  & 22.17 & &25.91 &23.44\\ 
% PAN &category  & \textbf{36.41}  &\textbf{40.58}  &\textbf{35.89} &&\textbf{24.79} & \textbf{17.39} & \textbf{26.14} & &\textbf{32.86} &\textbf{32.08}  \\  
% % \midrule
% MAttNet &supercategory &19.10  &  23.13&24.15&  &16.06 & 8.33 & 19.41 & &  10.08 & 12.77 \\
% PAN & supercategory&\textbf{22.83}&\textbf{31.25} &\textbf{25.32} & &\textbf{17.64} &\textbf{11.67} & \textbf{20.51}  &&\textbf{25.21}  & \textbf{26.37} \\ 
% % \bottomrule
% \end{tabular}
% }
% \end{center}
% \caption{Grounding accuracy and F1 score for grounding with category-based and supercategory-based selection. }
% \label{table:zsl}
% \end{table}

